Hidden in Plain Sight -- Class Competition Focuses Attribution Maps

Attribution methods reveal which input features a neural network uses for a prediction, adding transparency to their decisions. A common problem is that these attributions seem unspecific, highlighting both important and irrelevant features. We revisit the common attribution pipeline and observe that using logits as attribution target is a main cause of this phenomenon. We show that the solution is in plain sight: considering distributions of attributions over multiple classes using existing attribution methods yields specific and fine-grained attributions. On common benchmarks, including the grid-pointing game and randomization-based sanity checks, this improves the ability of 18 attribution methods across 7 architectures up to 2x, agnostic to model architecture.

==> defines.tex <==
% algorithm2e options
\SetKwComment{tcpas}{\{}{\}}
\SetCommentSty{textnormal}
\SetArgSty{textnormal}
\SetKwRepeat{Do}{do}{while}
\SetKw{False}{false}
\SetKw{True}{true}
\SetKw{Null}{null}
\SetKwInOut{Output}{output}
\SetKwInOut{Input}{input}
\SetKw{AND}{and}
\SetKw{OR}{or}
\SetKw{Continue}{continue}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> prettycolors/colors1.tex <==
\pgfplotscreateplotcyclelist{prcl-show-0}{
	{airforceblue} ,
	{aliceblue} ,
	{alizarin} ,
	{almond} ,
	{amaranth} ,
	{amber} , 
	{americanrose} ,
	{amethyst} ,
	{anti-flashwhite} ,
	{antiquebrass} ,
	{antiquefuchsia} ,
	{antiquewhite} ,
	{ao} ,
	{ao(english)} ,
	{applegreen} ,
	{apricot} ,
	{aqua} ,
	{aquamarine} ,
	{armygreen} ,
	{arsenic} ,
	{arylideyellow} ,
	{ashgrey} ,
	{asparagus} ,
	{atomictangerine} ,
	{auburn} ,
	{aureolin} ,
	{aurometalsaurus} ,
	{awesome} ,
	{azure(colorwheel)} ,
	{azure(web)(azuremist)} ,
	{babyblue} ,
	{babyblueeyes} ,
	{babypink} ,
	{ballblue} ,
	{bananamania} ,
	{bananayellow} ,
	{battleshipgrey} ,
	{bazaar} ,
	{beaublue} ,
	{beaver} ,
	{beige} ,
	{bisque} ,
	{bistre} ,
	{bittersweet} ,
	{black} ,
	{blanchedalmond} ,
	{bleudefrance} ,
	{blizzardblue} ,
	{blond} ,
	{blue} ,
}
\pgfplotscreateplotcyclelist{prcl-show-1}{
	{blue(munsell)} ,
	{blue(ncs)} ,
	{blue(pigment)} ,
	{blue(ryb)} ,
	{bluebell} ,
	{bluegray} ,
	{blue-green} ,
	{blue-violet} ,
	{blush} ,
	{bole} ,
	{bondiblue} ,
	{bostonuniversityred} ,
	{brandeisblue} ,
	{brass} ,
	{brickred} ,
	{brightcerulean} ,
	{brightgreen} ,
	{brightlavender} ,
	{brightmaroon} ,
	{brightpink} ,
	{brightturquoise} ,
	{brightube} ,
	{brilliantlavender} ,
	{brilliantrose} ,
	{brinkpink} ,
	{britishracinggreen} ,
	{bronze} ,
	{brown(traditional)} ,
	{brown(web)} ,
	{bubblegum} ,
	{bubbles} ,
	{buff} ,
	{bulgarianrose} ,
	{burgundy} ,
	{burlywood} ,
	{burntorange} ,
	{burntsienna} ,
	{burntumber} ,
	{byzantine} ,
	{byzantium} ,
	{cadet} ,
	{cadetblue} ,
	{cadetgrey} ,
	{cadmiumgreen} ,
	{cadmiumorange} ,
	{cadmiumred} ,
	{cadmiumyellow} ,
	{calpolypomonagreen} ,
	{cambridgeblue} ,
	{camel} ,
}
\pgfplotscreateplotcyclelist{prcl-show-2}{
	{camouflagegreen} ,
	{canaryyellow} ,
	{candyapplered} ,
	{candypink} ,
	{capri} ,
	{caputmortuum} ,
	{cardinal} ,
	{caribbeangreen} ,
	{carmine} ,
	{carminepink} ,
	{carminered} ,
	{carnationpink} ,
	{carnelian} ,
	{carolinablue} ,
	{carrotorange} ,
	{ceil} ,
	{celadon} ,
	{celestialblue} ,
	{cerise} ,
	{cerisepink} ,
	{cerulean} ,
	{ceruleanblue} ,
	{chamoisee} ,
	{champagne} ,
	{charcoal} ,
	{chartreuse(traditional)} ,
	{chartreuse(web)} ,
	{cherryblossompink} ,
	{chestnut} ,
	{chocolate(traditional)} ,
	{chocolate(web)} ,
	{chromeyellow} ,
	{cinereous} ,
	{cinnabar} ,
	{cinnamon} ,
	{citrine} ,
	{classicrose} ,
	{cobalt} ,
	{cocoabrown} ,
	{columbiablue} ,
	{coolblack} ,
	{coolgrey} ,
	{copper} ,
	{copperrose} ,
	{coquelicot} ,
	{coral} ,
	{coralpink} ,
	{coralred} ,
	{cordovan} ,
	{corn} ,
}
\pgfplotscreateplotcyclelist{prcl-show-3}{
	{cornellred} ,
	{cornflowerblue} ,
	{cornsilk} ,
	{cosmiclatte} ,
	{cottoncandy} ,
	{cream} ,
	{crimson} ,
	{crimsonglory} ,
	{cyan} ,
	{cyan(process)} ,
	{daffodil} ,
	{dandelion} ,
	{darkblue} ,
	{darkbrown} ,
	{darkbyzantium} ,
	{darkcandyapplered} ,
	{darkcerulean} ,
	{darkchampagne} ,
	{darkchestnut} ,
	{darkcoral} ,
	{darkcyan} ,
	{darkelectricblue} ,
	{darkgoldenrod} ,
	{darkgray} ,
	{darkgreen} ,
	{darkjunglegreen} ,
	{darkkhaki} ,
	{darklava} ,
	{darklavender} ,
	{darkmagenta} ,
	{darkmidnightblue} ,
	{darkolivegreen} ,
	{darkorange} ,
	{darkorchid} ,
	{darkpastelblue} ,
	{darkpastelgreen} ,
	{darkpastelpurple} ,
	{darkpastelred} ,
	{darkpink} ,
	{darkpowderblue} ,
	{darkraspberry} ,
	{darkred} ,
	{darksalmon} ,
	{darkscarlet} ,
	{darkseagreen} ,
	{darksienna} ,
	{darkslateblue} ,
	{darkslategray} ,
	{darkspringgreen} ,
	{darktan} ,
}
\pgfplotscreateplotcyclelist{prcl-show-4}{
	{darktangerine} ,
	{darktaupe} ,
	{darkterracotta} ,
	{darkturquoise} ,
	{darkviolet} ,
	{dartmouthgreen} ,
%	{davy\'sgrey} ,
	{debianred} ,
	{deepcarmine} ,
	{deepcarminepink} ,
	{deepcarrotorange} ,
	{deepcerise} ,
	{deepchampagne} ,
	{deepchestnut} ,
	{deepfuchsia} ,
	{deepjunglegreen} ,
	{deeplilac} ,
	{deepmagenta} ,
	{deeppeach} ,
	{deeppink} ,
	{deepsaffron} ,
	{deepskyblue} ,
	{denim} ,
	{desert} ,
	{desertsand} ,
	{dimgray} ,
	{dodgerblue} ,
	{dogwoodrose} ,
	{dollarbill} ,
	{drab} ,
	{dukeblue} ,
	{earthyellow} ,
	{ecru} ,
	{eggplant} ,
	{eggshell} ,
	{egyptianblue} ,
	{electricblue} ,
	{electriccrimson} ,
	{electriccyan} ,
	{electricgreen} ,
	{electricindigo} ,
	{electriclavender} ,
	{electriclime} ,
	{electricpurple} ,
	{electricultramarine} ,
	{electricviolet} ,
	{electricyellow} ,
	{emerald} ,
	{etonblue} ,
	{fallow} ,
}
\pgfplotscreateplotcyclelist{prcl-show-5}{
	{falured} ,
	{fandango} ,
	{fashionfuchsia} ,
	{fawn} ,
	{feldgrau} ,
	{ferngreen} ,
	{ferrarired} ,
	{fielddrab} ,
	{firebrick} ,
	{fireenginered} ,
	{flame} ,
	{flamingopink} ,
	{flavescent} ,
	{flax} ,
	{floralwhite} ,
	{fluorescentorange} ,
	{fluorescentpink} ,
	{fluorescentyellow} ,
	{folly} ,
	{forestgreen(traditional)} ,
	{forestgreen(web)} ,
	{frenchbeige} ,
	{frenchblue} ,
	{frenchlilac} ,
	{frenchrose} ,
	{fuchsia} ,
	{fuchsiapink} ,
	{fulvous} ,
	{fuzzywuzzy} ,
	{gainsboro} ,
	{gamboge} ,
	{ghostwhite} ,
	{ginger} ,
	{glaucous} ,
	{gold(metallic)} ,
	{gold(web)(golden)} ,
	{goldenbrown} ,
	{goldenpoppy} ,
	{goldenyellow} ,
	{goldenrod} ,
	{grannysmithapple} ,
	{gray} , 
%	{gray(html/cssgray)} ,
	{gray(x11gray)} ,
	{gray-asparagus} ,
	{green(colorwheel)(x11green)} , 
%	{green(html/cssgreen)} ,
	{green(munsell)} ,
	{green(ncs)} ,
	{green(pigment)} ,
}
\pgfplotscreateplotcyclelist{prcl-show-6}{
	{green(ryb)} ,
	{green-yellow} ,
	{grullo} ,
	{guppiegreen} ,
	{halayaube} ,
	{hanblue} ,
	{hanpurple} ,
	{hansayellow} ,
	{harlequin} ,
	{harvardcrimson} ,
	{harvestgold} ,
	{heartgold} ,
	{heliotrope} ,
	{hollywoodcerise} ,
	{honeydew} ,
	%{hooker\'sgreen} ,
	{hotmagenta} ,
	{hotpink} ,
	{huntergreen} ,
	{iceberg} ,
	{icterine} ,
	{inchworm} ,
	{indiagreen} ,
	{indianred} ,
	{indianyellow} ,
	{indigo(dye)} ,
	{indigo(web)} ,
	{internationalkleinblue} ,
	{internationalorange} ,
	{iris} ,
	{isabelline} ,
	{islamicgreen} ,
	{ivory} ,
	{jade} ,
	{jasper} ,
	{jazzberryjam} ,
	{jonquil} ,
	{junebud} ,
	{junglegreen} ,
	{kellygreen} ,
%	{khaki(html/css)(khaki)} ,
	{khaki(x11)(lightkhaki)} ,
	{lasallegreen} ,
	{languidlavender} ,
	{lapislazuli} ,
	{laserlemon} ,
	{lava} ,
	{lavender(floral)} ,
	{lavender(web)} ,
	{lavenderblue} ,
}
\pgfplotscreateplotcyclelist{prcl-show-7}{
	{lavenderblush} ,
	{lavendergray} ,
	{lavenderindigo} ,
	{lavendermagenta} ,
	{lavendermist} ,
	{lavenderpink} ,
	{lavenderpurple} ,
	{lavenderrose} ,
	{lawngreen} ,
	{lemon} ,
	{lemonchiffon} ,
	{lightapricot} ,
	{lightblue} ,
	{lightbrown} ,
	{lightcarminepink} ,
	{lightcoral} ,
	{lightcornflowerblue} ,
	{lightcyan} ,
	{lightfuchsiapink} ,
	{lightgoldenrodyellow} ,
	{lightgray} ,
	{lightgreen} ,
	{lightkhaki} ,
	{lightmauve} ,
	{lightpastelpurple} ,
	{lightpink} ,
	{lightsalmon} ,
	{lightsalmonpink} ,
	{lightseagreen} ,
	{lightskyblue} ,
	{lightslategray} ,
	{lighttaupe} ,
	{lightthulianpink} ,
	{lightyellow} ,
	{lilac} ,
	{lime(colorwheel)} ,
	{lime(web)(x11green)} ,
	{limegreen} ,
	{lincolngreen} ,
	{linen} ,
	{liver} ,
	{lust} ,
	{macaroniandcheese} ,
	{magenta} ,
	{magenta(dye)} ,
	{magenta(process)} ,
	{magicmint} ,
	{magnolia} ,
	{mahogany} ,
	{maize} ,
}
\pgfplotscreateplotcyclelist{prcl-show-8}{
	{majorelleblue} ,
	{malachite} ,
	{manatee} ,
	{mangotango} ,
%	{maroon(html/css)} ,
	{maroon(x11)} ,
	{mauve} ,
	{mauvetaupe} ,
	{mauvelous} ,
	{mayablue} ,
	{meatbrown} ,
	{mediumaquamarine} ,
	{mediumblue} ,
	{mediumcandyapplered} ,
	{mediumcarmine} ,
	{mediumchampagne} ,
	{mediumelectricblue} ,
	{mediumjunglegreen} ,
	{mediumlavendermagenta} ,
	{mediumorchid} ,
	{mediumpersianblue} ,
	{mediumpurple} ,
	{mediumred-violet} ,
	{mediumseagreen} ,
	{mediumslateblue} ,
	{mediumspringbud} ,
	{mediumspringgreen} ,
	{mediumtaupe} ,
	{mediumtealblue} ,
	{mediumturquoise} ,
	{mediumviolet-red} ,
	{melon} ,
	{midnightblue} ,
	{midnightgreen(eaglegreen)} ,
	{mikadoyellow} ,
	{mint} ,
	{mintcream} ,
	{mintgreen} ,
	{mistyrose} ,
	{moccasin} ,
	{modebeige} ,
	{moonstoneblue} ,
	{mordantred19} ,
	{mossgreen} ,
	{mountainmeadow} ,
	{mountbattenpink} ,
	{mulberry} ,
	{mustard} ,
	{myrtle} ,
	{msugreen} ,
}
\pgfplotscreateplotcyclelist{prcl-show-9}{
	{nadeshikopink} ,
	{napiergreen} ,
	{naplesyellow} ,
	{navajowhite} ,
	{navyblue} ,
	{neoncarrot} ,
	{neonfuchsia} ,
	{neongreen} ,
	{non-photoblue} ,
	{oceanboatblue} ,
	{ochre} ,
	{officegreen} ,
	{oldgold} ,
	{oldlace} ,
	{oldlavender} ,
	{oldmauve} ,
	{oldrose} ,
	{olive} ,
	{olivedrab(web)(olivedrab3)} ,
	{olivedrab7} ,
	{olivine} ,
	{onyx} ,
	{operamauve} ,
	{orange(colorwheel)} ,
	{orange(ryb)} ,
	{orange(webcolor)} ,
	{orangepeel} ,
	{orange-red} ,
	{orchid} ,
	{otterbrown} ,
	{outerspace} ,
	{outrageousorange} ,
	{oxfordblue} ,
	{oucrimsonred} ,
	{pakistangreen} ,
	{palatinateblue} ,
	{palatinatepurple} ,
	{paleaqua} ,
	{paleblue} ,
	{palebrown} ,
	{palecarmine} ,
	{palecerulean} ,
	{palechestnut} ,
	{palecopper} ,
	{palecornflowerblue} ,
	{palegold} ,
	{palegoldenrod} ,
	{palegreen} ,
	{palemagenta} ,
	{palepink} ,
}
\pgfplotscreateplotcyclelist{prcl-show-10}{
	{paleplum} ,
	{palered-violet} ,
	{palerobineggblue} ,
	{palesilver} ,
	{palespringbud} ,
	{paletaupe} ,
	{paleviolet-red} ,
	{pansypurple} ,
	{papayawhip} ,
	{parisgreen} ,
	{pastelblue} ,
	{pastelbrown} ,
	{pastelgray} ,
	{pastelgreen} ,
	{pastelmagenta} ,
	{pastelorange} ,
	{pastelpink} ,
	{pastelpurple} ,
	{pastelred} ,
	{pastelviolet} ,
	{pastelyellow} ,
	{patriarch} ,
%	{payne\'sgrey} ,
	{peach} ,
	{peach-orange} ,
	{peachpuff} ,
	{peach-yellow} ,
	{pear} ,
	{pearl} ,
	{peridot} ,
	{periwinkle} ,
	{persianblue} ,
	{persiangreen} ,
	{persianindigo} ,
	{persianorange} ,
	{peru} ,
	{persianpink} ,
	{persianplum} ,
	{persianred} ,
	{persianrose} ,
	{persimmon} ,
	{phlox} ,
	{phthaloblue} ,
	{phthalogreen} ,
	{piggypink} ,
	{pinegreen} ,
	{pink} ,
	{pink-orange} ,
	{pinkpearl} ,
	{pinksherbet} ,
}
\pgfplotscreateplotcyclelist{prcl-show-11}{
	{pistachio} ,
	{platinum} ,
	{plum(traditional)} ,
	{plum(web)} ,
	{portlandorange} ,
	{powderblue(web)} ,
	{princetonorange} ,
	{prune} ,
	{prussianblue} ,
	{psychedelicpurple} ,
	{puce} ,
	{pumpkin} ,
%	{purple(html/css)} ,
	{purple(munsell)} ,
	{purple(x11)} ,
	{purpleheart} ,
	{purplemountainmajesty} ,
	{purplepizzazz} ,
	{purpletaupe} ,
	{radicalred} ,
	{raspberry} ,
	{raspberryglace} ,
	{raspberrypink} ,
	{raspberryrose} ,
	{rawumber} ,
	{razzledazzlerose} ,
	{razzmatazz} ,
	{red} ,
	{red(munsell)} ,
	{red(ncs)} ,
	{red(pigment)} ,
	{red(ryb)} ,
	{red-brown} ,
	{red-violet} ,
	{redwood} ,
	{regalia} ,
	{richblack} ,
	{richbrilliantlavender} ,
	{richcarmine} ,
	{richelectricblue} ,
	{richlavender} ,
	{richlilac} ,
	{richmaroon} ,
	{riflegreen} ,
	{robineggblue} ,
	{rose} ,
	{rosebonbon} ,
	{roseebony} ,
	{rosegold} ,
	{rosemadder} ,
}
\pgfplotscreateplotcyclelist{prcl-show-12}{
	{rosepink} ,
	{rosequartz} ,
	{rosetaupe} ,
	{rosevale} ,
	{rosewood} ,
	{rossocorsa} ,
	{rosybrown} ,
	{royalazure} ,
	{royalblue(traditional)} ,
	{royalblue(web)} ,
	{royalfuchsia} ,
	{royalpurple} ,
	{ruby} ,
	{ruddy} ,
	{ruddybrown} ,
	{ruddypink} ,
	{rufous} ,
	{russet} ,
	{rust} ,
	{sacramentostategreen} ,
	{saddlebrown} ,
	{safetyorange(blazeorange)} ,
	{saffron} ,
%	{st.patrick\'sblue} ,
	{salmon} ,
	{salmonpink} ,
	{sand} ,
	{sanddune} ,
	{sandstorm} ,
	{sandybrown} ,
	{sandytaupe} ,
	{sangria} ,
	{sapgreen} ,
	{sapphire} ,
	{satinsheengold} ,
	{scarlet} ,
	{schoolbusyellow} ,
%	{screamin\'green} ,
	{seagreen} ,
	{sealbrown} ,
	{seashell} ,
	{selectiveyellow} ,
	{sepia} ,
	{shadow} ,
	{shamrockgreen} ,
	{shockingpink} ,
	{sienna} ,
	{silver} ,
	{sinopia} ,
	{skobeloff} ,
}
\pgfplotscreateplotcyclelist{prcl-show-13}{
	{skyblue} ,
	{skymagenta} ,
	{slateblue} ,
	{slategray} ,
	{smalt(darkpowderblue)} ,
	{smokeytopaz} ,
	{smokyblack} ,
	{snow} ,
	{spirodiscoball} ,
	{splashedwhite} ,
	{springbud} ,
	{springgreen} ,
	{steelblue} ,
	{stildegrainyellow} ,
	{straw} ,
	{sunglow} ,
	{sunset} ,
	{tan} ,
	{tangelo} ,
	{tangerine} ,
	{tangerineyellow} ,
	{taupe} ,
	{taupegray} ,
	{teagreen} ,
	{tearose(orange)} ,
	{tearose(rose)} ,
	{teal} ,
	{tealblue} ,
	{tealgreen} ,
%	{tenné(tawny)} ,
	{terracotta} ,
	{thistle} ,
	{thulianpink} ,
	{ticklemepink} ,
	{tiffanyblue} ,
%	{tiger\'seye} ,
	{timberwolf} ,
	{titaniumyellow} ,
	{tomato} ,
	{toolbox} ,
	{tractorred} ,
	{trolleygrey} ,
	{tropicalrainforest} ,
	{trueblue} ,
	{tuftsblue} ,
	{tumbleweed} ,
	{turkishrose} ,
	{turquoise} ,
	{turquoiseblue} ,
	{turquoisegreen} ,
}
\pgfplotscreateplotcyclelist{prcl-show-14}{
	{tuscanred} ,
	{twilightlavender} ,
	{tyrianpurple} ,
	{uablue} ,
	{uared} ,
	{ube} ,
	{uclablue} ,
	{uclagold} ,
	{ufogreen} ,
	{ultramarine} ,
	{ultramarineblue} ,
	{ultrapink} ,
	{umber} ,
	{unitednationsblue} ,
	{unmellowyellow} ,
	{upforestgreen} ,
	{upmaroon} ,
	{upsdellred} ,
	{urobilin} ,
	{usccardinal} ,
	{uscgold} ,
	{utahcrimson} ,
	{vanilla} ,
	{vegasgold} ,
	{venetianred} ,
	{verdigris} ,
	{vermilion} ,
	{veronica} ,
	{violet} ,
	{violet(colorwheel)} ,
	{violet(ryb)} ,
	{violet(web)} ,
	{viridian} ,
	{vividauburn} ,
	{vividburgundy} ,
	{vividcerise} ,
	{vividtangerine} ,
	{vividviolet} ,
	{warmblack} ,
	{wenge} ,
	{wheat} ,
	{white} ,
	{whitesmoke} ,
	{wildblueyonder} ,
	{wildstrawberry} ,
	{wildwatermelon} ,
	{wisteria} ,
	{xanadu} ,
	{yaleblue} ,
	{yellow} ,
	{yellow(munsell)} ,
	{yellow(ncs)} ,
	{yellow(process)} ,
	{yellow(ryb)} ,
	{yellow-green} ,
	{zaffre} ,
	{zinnwalditebrown} ,
}
 
\tikzstyle{mark_sel} = [pengublue, only marks, mark=*,mark options={fill opacity=0.70}, mark size=1.5, line width =.7pt]

\tikzstyle{mark_usel} =[gray!40,  mark=*,mark options={fill opacity=0.40}, only marks, mark size=1.5, line width =.7pt]

\tikzstyle{line_usel}= [pengublue, opacity=.7, line width = 1.7pt]

\tikzstyle{line_sel}= [mambacolor2,opacity=.9, line width = 1.7pt]

\tikzstyle{line_oracle} =[gray, densely dashed, opacity=.6, line width = 1.7pt]





==> prettycolors/colors2.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-0,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
	\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{airforceblue, aliceblue, alizarin, almond, amaranth, amber, %amber(sae/ece),
 americanrose, amethyst, anti-flashwhite, antiquebrass, antiquefuchsia, antiquewhite, ao, ao(english), applegreen, apricot, aqua, aquamarine, armygreen, arsenic, arylideyellow, ashgrey, asparagus, atomictangerine, auburn, aureolin, aurometalsaurus, awesome, azure(colorwheel), azure(web)(azuremist), babyblue, babyblueeyes, babypink, ballblue, bananamania, bananayellow, battleshipgrey, bazaar, beaublue, beaver, beige, bisque, bistre, bittersweet, black, blanchedalmond, bleudefrance, blizzardblue, blond, blue}
\end{axis}
\end{tikzpicture}
\end{figure}


\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-1,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{blue(munsell), blue(ncs), blue(pigment), blue(ryb), bluebell, bluegray, blue-green, blue-violet, blush, bole, bondiblue, bostonuniversityred, brandeisblue, brass, brickred, brightcerulean, brightgreen, brightlavender, brightmaroon, brightpink, brightturquoise, brightube, brilliantlavender, brilliantrose, brinkpink, britishracinggreen, bronze, brown(traditional), brown(web), bubblegum, bubbles, buff, bulgarianrose, burgundy, burlywood, burntorange, burntsienna, burntumber, byzantine, byzantium, cadet, cadetblue, cadetgrey, cadmiumgreen, cadmiumorange, cadmiumred, cadmiumyellow, calpolypomonagreen, cambridgeblue, camel}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-2,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{camouflagegreen, canaryyellow, candyapplered, candypink, capri, caputmortuum, cardinal, caribbeangreen, carmine, carminepink, carminered, carnationpink, carnelian, carolinablue, carrotorange, ceil, celadon, celestialblue, cerise, cerisepink, cerulean, ceruleanblue, chamoisee, champagne, charcoal, chartreuse(traditional), chartreuse(web), cherryblossompink, chestnut, chocolate(traditional), chocolate(web), chromeyellow, cinereous, cinnabar, cinnamon, citrine, classicrose, cobalt, cocoabrown, columbiablue, coolblack, coolgrey, copper, copperrose, coquelicot, coral, coralpink, coralred, cordovan, corn}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
	\begin{axis}[ pretty line,
	pretty spacy,
	cycle list name = prcl-show-3,
	ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
	legend pos=north east, legend columns=2, 
	legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
	xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
	ymin=0, ymax=100,  ] 
	\pgfplotsinvokeforeach{1, ..., 50}{ 
		\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
	};
	\legend{cornellred, cornflowerblue, cornsilk, cosmiclatte, cottoncandy, cream, crimson, crimsonglory, cyan, cyan(process), daffodil, dandelion, darkblue, darkbrown, darkbyzantium, darkcandyapplered, darkcerulean, darkchampagne, darkchestnut, darkcoral, darkcyan, darkelectricblue, darkgoldenrod, darkgray, darkgreen, darkjunglegreen, darkkhaki, darklava, darklavender, darkmagenta, darkmidnightblue, darkolivegreen, darkorange, darkorchid, darkpastelblue, darkpastelgreen, darkpastelpurple, darkpastelred, darkpink, darkpowderblue, darkraspberry, darkred, darksalmon, darkscarlet, darkseagreen, darksienna, darkslateblue, darkslategray, darkspringgreen, darktan}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-4,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{darktangerine, darktaupe, darkterracotta, darkturquoise, darkviolet, dartmouthgreen, %davy\'sgrey, 
	debianred, deepcarmine, deepcarminepink, deepcarrotorange, deepcerise, deepchampagne, deepchestnut, deepfuchsia, deepjunglegreen, deeplilac, deepmagenta, deeppeach, deeppink, deepsaffron, deepskyblue, denim, desert, desertsand, dimgray, dodgerblue, dogwoodrose, dollarbill, drab, dukeblue, earthyellow, ecru, eggplant, eggshell, egyptianblue, electricblue, electriccrimson, electriccyan, electricgreen, electricindigo, electriclavender, electriclime, electricpurple, electricultramarine, electricviolet, electricyellow, emerald, etonblue, fallow}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-5,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 48}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{falured, fandango, fashionfuchsia, fawn, feldgrau, ferngreen, ferrarired, fielddrab, firebrick, fireenginered, flame, flamingopink, flavescent, flax, floralwhite, fluorescentorange, fluorescentpink, fluorescentyellow, folly, forestgreen(traditional), forestgreen(web), frenchbeige, frenchblue, frenchlilac, frenchrose, fuchsia, fuchsiapink, fulvous, fuzzywuzzy, gainsboro, gamboge, ghostwhite, ginger, glaucous, gold(metallic), gold(web)(golden), goldenbrown, goldenpoppy, goldenyellow, goldenrod, grannysmithapple, gray,   %gray(html/cssgray), 
gray(x11gray), gray-asparagus, green(colorwheel)(x11green),  %green(html/cssgreen),
green(munsell), green(ncs), green(pigment)}
\end{axis}
\end{tikzpicture}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

==> prettycolors/colors3.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-6,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 48}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{green(ryb), green-yellow, grullo, guppiegreen, halayaube, hanblue, hanpurple, hansayellow, harlequin, harvardcrimson, harvestgold, heartgold, heliotrope, hollywoodcerise, honeydew, %hooker\'sgreen,
	 hotmagenta, hotpink, huntergreen, iceberg, icterine, inchworm, indiagreen, indianred, indianyellow, indigo(dye), indigo(web), internationalkleinblue, internationalorange, iris, isabelline, islamicgreen, ivory, jade, jasper, jazzberryjam, jonquil, junebud, junglegreen, kellygreen, 
%khaki(html/css)(khaki), 
khaki(x11)(lightkhaki), lasallegreen, languidlavender, lapislazuli, laserlemon, lava, lavender(floral), lavender(web), lavenderblue}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-7,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{lavenderblush, lavendergray, lavenderindigo, lavendermagenta, lavendermist, lavenderpink, lavenderpurple, lavenderrose, lawngreen, lemon, lemonchiffon, lightapricot, lightblue, lightbrown, lightcarminepink, lightcoral, lightcornflowerblue, lightcyan, lightfuchsiapink, lightgoldenrodyellow, lightgray, lightgreen, lightkhaki, lightmauve, lightpastelpurple, lightpink, lightsalmon, lightsalmonpink, lightseagreen, lightskyblue, lightslategray, lighttaupe, lightthulianpink, lightyellow, lilac, lime(colorwheel), lime(web)(x11green), limegreen, lincolngreen, linen, liver, lust, macaroniandcheese, magenta, magenta(dye), magenta(process), magicmint, magnolia, mahogany, maize}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-8,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 49}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{majorelleblue, malachite, manatee, mangotango, %maroon(html/css),
maroon(x11), mauve, mauvetaupe, mauvelous, mayablue, meatbrown, mediumaquamarine, mediumblue, mediumcandyapplered, mediumcarmine, mediumchampagne, mediumelectricblue, mediumjunglegreen, mediumlavendermagenta, mediumorchid, mediumpersianblue, mediumpurple, mediumred-violet, mediumseagreen, mediumslateblue, mediumspringbud, mediumspringgreen, mediumtaupe, mediumtealblue, mediumturquoise, mediumviolet-red, melon, midnightblue, midnightgreen(eaglegreen), mikadoyellow, mint, mintcream, mintgreen, mistyrose, moccasin, modebeige, moonstoneblue, mordantred19, mossgreen, mountainmeadow, mountbattenpink, mulberry, mustard, myrtle, msugreen}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-9,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 50}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{nadeshikopink, napiergreen, naplesyellow, navajowhite, navyblue, neoncarrot, neonfuchsia, neongreen, non-photoblue, oceanboatblue, ochre, officegreen, oldgold, oldlace, oldlavender, oldmauve, oldrose, olive, olivedrab(web)(olivedrab3), olivedrab7, olivine, onyx, operamauve, orange(colorwheel), orange(ryb), orange(webcolor), orangepeel, orange-red, orchid, otterbrown, outerspace, outrageousorange, oxfordblue, oucrimsonred, pakistangreen, palatinateblue, palatinatepurple, paleaqua, paleblue, palebrown, palecarmine, palecerulean, palechestnut, palecopper, palecornflowerblue, palegold, palegoldenrod, palegreen, palemagenta, palepink}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-10,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 49}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{paleplum, palered-violet, palerobineggblue, palesilver, palespringbud, paletaupe, paleviolet-red, pansypurple, papayawhip, parisgreen, pastelblue, pastelbrown, pastelgray, pastelgreen, pastelmagenta, pastelorange, pastelpink, pastelpurple, pastelred, pastelviolet, pastelyellow, patriarch, %payne\'sgrey,
	 peach, peach-orange, peachpuff, peach-yellow, pear, pearl, peridot, periwinkle, persianblue, persiangreen, persianindigo, persianorange, peru, persianpink, persianplum, persianred, persianrose, persimmon, phlox, phthaloblue, phthalogreen, piggypink, pinegreen, pink, pink-orange, pinkpearl, pinksherbet}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[ pretty line,
pretty spacy,
cycle list name = prcl-show-11,
ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
legend pos=north east, legend columns=2, 
legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
ymin=0, ymax=100,  ] 
\pgfplotsinvokeforeach{1, ..., 49}{ 
\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
};
\legend{pistachio, platinum, plum(traditional), plum(web), portlandorange, powderblue(web), princetonorange, prune, prussianblue, psychedelicpurple, puce, pumpkin, 
purple(munsell), purple(x11), purpleheart, purplemountainmajesty, purplepizzazz, purpletaupe, radicalred, raspberry, raspberryglace, raspberrypink, raspberryrose, rawumber, razzledazzlerose, razzmatazz, red, red(munsell), red(ncs), red(pigment), red(ryb), red-brown, red-violet, redwood, regalia, richblack, richbrilliantlavender, richcarmine, richelectricblue, richlavender, richlilac, richmaroon, riflegreen, robineggblue, rose, rosebonbon, roseebony, rosegold, rosemadder}
\end{axis}
\end{tikzpicture}
\end{figure}


==> prettycolors/colors4.tex <==
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
	\begin{axis}[ pretty line,
	pretty spacy,
	cycle list name = prcl-show-12,
	ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
	legend pos=north east, legend columns=2, 
	legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
	xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
	ymin=0, ymax=100,  ] 
	\pgfplotsinvokeforeach{1, ..., 48}{ 
		\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
	};
	\legend{rosepink, rosequartz, rosetaupe, rosevale, rosewood, rossocorsa, rosybrown, royalazure, royalblue(traditional), royalblue(web), royalfuchsia, royalpurple, ruby, ruddy, ruddybrown, ruddypink, rufous, russet, rust, sacramentostategreen, saddlebrown, safetyorange(blazeorange), saffron, %st.patrick\'sblue, 
		salmon, salmonpink, sand, sanddune, sandstorm, sandybrown, sandytaupe, sangria, sapgreen, sapphire, satinsheengold, scarlet, schoolbusyellow,% screamin\'green, 
		seagreen, sealbrown, seashell, selectiveyellow, sepia, shadow, shamrockgreen, shockingpink, sienna, silver, sinopia, skobeloff}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
	\begin{axis}[ pretty line,
	pretty spacy,
	cycle list name = prcl-show-13,
	ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
	legend pos=north east, legend columns=2, 
	legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
	xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
	ymin=0, ymax=100,  ] 
	\pgfplotsinvokeforeach{1, ..., 48}{ 
		\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
	};
\legend{skyblue, skymagenta, slateblue, slategray, smalt(darkpowderblue), smokeytopaz, smokyblack, snow, spirodiscoball, splashedwhite, springbud, springgreen, steelblue, stildegrainyellow, straw, sunglow, sunset, tan, tangelo, tangerine, tangerineyellow, taupe, taupegray, teagreen, tearose(orange), tearose(rose), teal, tealblue, tealgreen, % tenné(tawny),
	 terracotta, thistle, thulianpink, ticklemepink, tiffanyblue, % tiger\'seye,
	 timberwolf, titaniumyellow, tomato, toolbox, tractorred, trolleygrey, tropicalrainforest, trueblue, tuftsblue, tumbleweed, turkishrose, turquoise, turquoiseblue, turquoisegreen}
\end{axis}
\end{tikzpicture}
\end{figure}
\begin{figure}[h]
	\centering
	\begin{tikzpicture}
	\begin{axis}[ pretty line,
	pretty spacy,
	cycle list name = prcl-show-14,
	ylabel = {x}, xlabel = {y},   height = 8 cm, width = 10 cm,
	legend pos=north east, legend columns=2, 
	legend style={nodes={scale=0.65, transform shape}, at={(1.05, 1.05)}, anchor=north west}, 
	xmin=0, xmax=100, % xtick={0, 0.25, 0.5, 0.75, 1}, 
	ymin=0, ymax=100,  ] 
	\pgfplotsinvokeforeach{1, ..., 57}{ 
		\addplot+[domain=1:100, line width = 1.2, opacity=.8]  {2 *  #1+.1*x};
	};
\legend{tuscanred, twilightlavender, tyrianpurple, uablue, uared, ube, uclablue, uclagold, ufogreen, ultramarine, ultramarineblue, ultrapink, umber, unitednationsblue, unmellowyellow, upforestgreen, upmaroon, upsdellred, urobilin, usccardinal, uscgold, utahcrimson, vanilla, vegasgold, venetianred, verdigris, vermilion, veronica, violet, violet(colorwheel), violet(ryb), violet(web), viridian, vividauburn, vividburgundy, vividcerise, vividtangerine, vividviolet, warmblack, wenge, wheat, white, whitesmoke, wildblueyonder, wildstrawberry, wildwatermelon, wisteria, xanadu, yaleblue, yellow, yellow(munsell), yellow(ncs), yellow(process), yellow(ryb), yellow-green, zaffre, zinnwalditebrown}
\end{axis}
\end{tikzpicture}
\end{figure}



==> prettycolors/eda-more-colors.tex <==

\definecolor{color(mmci)}{cmyk}{1,0.4,0,0}
\definecolor{color(cispa)}{rgb}{0.008,0.356,0.584}
\definecolor{color(helmholtzblue)}{RGB}{0, 90, 160}
\definecolor{color(helmholtzgreen)}{RGB}{140, 180, 35}

\definecolor{wong-blue}{RGB}{0, 114, 178}
\definecolor{wong-orange}{RGB}{230, 159, 0}
\definecolor{wong-green}{RGB}{0, 158, 115}
\definecolor{wong-reddishpurple}{RGB}{204, 121, 167}
\definecolor{wong-skyblue}{RGB}{86, 180, 233}
\definecolor{wong-vermillion}{RGB}{213, 94, 0}
\definecolor{wong-yellow}{RGB}{240, 228, 66}

% https://personal.sron.nl/~pault/#sec:qualitative
\definecolor{tol-q-bright-blue}{HTML}{4477AA}
\definecolor{tol-q-bright-cyan}{HTML}{66CCEE}
\definecolor{tol-q-bright-green}{HTML}{228833}
\definecolor{tol-q-bright-yellow}{HTML}{CCBB44}
\definecolor{tol-q-bright-red}{HTML}{EE6677}
\definecolor{tol-q-bright-purple}{HTML}{AA3377}
\definecolor{tol-q-bright-grey}{HTML}{BBBBBB}

\definecolor{tol-q-high-contrast-white}{HTML}{FFFFFF}
\definecolor{tol-q-high-contrast-yellow}{HTML}{DDAA33}
\definecolor{tol-q-high-contrast-red}{HTML}{BB5566}
\definecolor{tol-q-high-contrast-blue}{HTML}{004488}
\definecolor{tol-q-high-contrast-black}{HTML}{000000}

\definecolor{tol-q-vibrant-blue}{HTML}{0077BB}
\definecolor{tol-q-vibrant-cyan}{HTML}{33BBEE}
\definecolor{tol-q-vibrant-teal}{HTML}{009988}
\definecolor{tol-q-vibrant-orange}{HTML}{EE7733}
\definecolor{tol-q-vibrant-red}{HTML}{CC3311}
\definecolor{tol-q-vibrant-magenta}{HTML}{EE3377}
\definecolor{tol-q-vibrant-grey}{HTML}{BBBBBB}

\definecolor{tol-q-muted-indigo}{HTML}{332288}
\definecolor{tol-q-muted-cyan}{HTML}{88CCEE}
\definecolor{tol-q-muted-teal}{HTML}{44AA99}
\definecolor{tol-q-muted-green}{HTML}{117733 }
\definecolor{tol-q-muted-olive}{HTML}{999933}
\definecolor{tol-q-muted-sand}{HTML}{DDCC77}
\definecolor{tol-q-muted-rose}{HTML}{CC6677}
\definecolor{tol-q-muted-wine}{HTML}{882255}
\definecolor{tol-q-muted-purple}{HTML}{AA4499}
\definecolor{tol-q-muted-pale-grey}{HTML}{DDDDDD}

\definecolor{tol-mark-pale-blue}{HTML}{BBCCEE}
\definecolor{tol-mark-pale-cyan}{HTML}{CCEEFF}
\definecolor{tol-mark-pale-green}{HTML}{CCDDAA}
\definecolor{tol-mark-pale-yellow}{HTML}{EEEEBB}
\definecolor{tol-mark-pale-red}{HTML}{FFCCCC}
\definecolor{tol-mark-pale-grey}{HTML}{DDDDDD}

\definecolor{tol-mark-dark-blue}{HTML}{222255}
\definecolor{tol-mark-dark-cyan}{HTML}{225555}
\definecolor{tol-mark-dark-green}{HTML}{225522}
\definecolor{tol-mark-dark-yellow}{HTML}{666633}
\definecolor{tol-mark-dark-red}{HTML}{663333}
\definecolor{tol-mark-pale-grey}{HTML}{555555}

\definecolor{tol-q-light-blue}{HTML}{77AADD}
\definecolor{tol-q-light-cyan}{HTML}{99DDFF}
\definecolor{tol-q-light-mint}{HTML}{44BB99}
\definecolor{tol-q-light-pear}{HTML}{BBCC33}
\definecolor{tol-q-light-olive}{HTML}{AAAA00}
\definecolor{tol-q-light-yellow}{HTML}{EEDD88}
\definecolor{tol-q-light-orange}{HTML}{EE8866}
\definecolor{tol-q-light-pink}{HTML}{FFAABB}
\definecolor{tol-q-light-pale-grey}{HTML}{DDDDDD}

\colorlet{color(ourmethod)}{tol-q-muted-indigo} 	
\colorlet{color(ourmethodsemi)}{tol-q-muted-indigo} 	
\colorlet{color(asso)}{tol-q-muted-cyan} 	
\colorlet{color(grecond)}{tol-q-muted-teal} 	
\colorlet{color(nmf)}{tol-q-muted-green} 	
\colorlet{color(nmfr)}{tol-q-muted-olive} 	
\colorlet{color(sofa)}{tol-q-muted-sand} 	
\colorlet{color(binaps)}{tol-q-muted-rose} 	
\colorlet{color(pimp)}{tol-q-muted-wine}

\definecolor{TSneColor(0.0)}{RGB}{136, 204, 238}
\definecolor{TSneColor(1.0)}{RGB}{117, 194, 214}
\definecolor{TSneColor(2.0)}{RGB}{98, 185, 190}
\definecolor{TSneColor(3.0)}{RGB}{79, 175, 166}
\definecolor{TSneColor(4.0)}{RGB}{62, 164, 140}
\definecolor{TSneColor(5.0)}{RGB}{47, 149, 112}
\definecolor{TSneColor(6.0)}{RGB}{33, 135, 83}
\definecolor{TSneColor(7.0)}{RGB}{19, 121, 54}
\definecolor{TSneColor(8.0)}{RGB}{26, 98, 72}
\definecolor{TSneColor(9.0)}{RGB}{35, 74, 96}
\definecolor{TSneColor(10.0)}{RGB}{45, 50, 120}
\definecolor{TSneColor(11.0)}{RGB}{67, 50, 134}
\definecolor{TSneColor(12.0)}{RGB}{115, 98, 130}
\definecolor{TSneColor(13.0)}{RGB}{163, 146, 125}
\definecolor{TSneColor(14.0)}{RGB}{210, 193, 120}
\definecolor{TSneColor(15.0)}{RGB}{206, 193, 104}
\definecolor{TSneColor(16.0)}{RGB}{187, 178, 85}
\definecolor{TSneColor(17.0)}{RGB}{168, 164, 66}
\definecolor{TSneColor(18.0)}{RGB}{156, 150, 55}
\definecolor{TSneColor(19.0)}{RGB}{171, 135, 74}
\definecolor{TSneColor(20.0)}{RGB}{185, 121, 94}
\definecolor{TSneColor(21.0)}{RGB}{199, 107, 113}
\definecolor{TSneColor(22.0)}{RGB}{191, 89, 113}
\definecolor{TSneColor(23.0)}{RGB}{172, 70, 103}
\definecolor{TSneColor(24.0)}{RGB}{153, 51, 94}
\definecolor{TSneColor(25.0)}{RGB}{137, 35, 87}
\definecolor{TSneColor(26.0)}{RGB}{147, 45, 106}
\definecolor{TSneColor(27.0)}{RGB}{156, 54, 125}
\definecolor{TSneColor(28.0)}{RGB}{166, 64, 144}
\definecolor{TSneColor(29.0)}{RGB}{178, 92, 164}
\definecolor{TSneColor(30.0)}{RGB}{192, 135, 183}
\definecolor{TSneColor(31.0)}{RGB}{207, 178, 202}
\definecolor{TSneColor(32.0)}{RGB}{221, 221, 221}

\definecolor{clust1col}{RGB}{101,66,134}
\definecolor{clust2col}{HTML}{0891b2}
\definecolor{nipsvio}{RGB}{101,66,134}
\definecolor{testblue}{HTML}{06b6d4}

\definecolor{s0}{HTML}{ff9b02} % a
\definecolor{s1}{HTML}{F9D923} % b
\definecolor{s2}{HTML}{134e6f} % c
\definecolor{s3}{HTML}{ff6150} % d
\definecolor{s4}{HTML}{1ac0c6} % e
\definecolor{s5}{HTML}{36AE7C} % f

\definecolor{e0}{HTML}{ff6150}
\definecolor{e1}{HTML}{1ac0c6}
\definecolor{e2}{HTML}{F9D923}
\definecolor{e3}{HTML}{36AE7C}
\definecolor{e4}{HTML}{134e6f}
\definecolor{e5}{HTML}{ff6150}
\definecolor{e6}{HTML}{1ac0c6}
\definecolor{e7}{HTML}{ff9b02}

\definecolor{abst1}{HTML}{E4C1F9}
\definecolor{abst2}{HTML}{4F7CAC}
\definecolor{abst3}{HTML}{9EEFE5}
\definecolor{abst4}{HTML}{541388} 

\definecolor{mygreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{mygray}{rgb}{0.3, 0.3, 0.3}

\newcommand{\cakecolor}{mambacolor2}
\newcommand{\sqscolor}{mambacolor1}
\newcommand{\bidecolor}{mambacolor3}
\newcommand{\sciscolor}{mambacolor4}
\newcommand{\ismcolor}{mambacolor5}
\newcommand{\cutecolor}{mambacolor6}
\newcommand{\tentcolor}{mambacolor7}
\newcommand{\nullmodelcolor}{black}
\newcommand{\plantedmodellcolor}{mygreen}
\definecolor{variolila}{RGB}{115,100,137}
\definecolor{lilacgray}{RGB}{152,150,164}
\definecolor{red1}{RGB}{201,59,69}
\definecolor{cc1}{rgb}{0.59, 0.78, 0.64}
\definecolor{niceblue}{RGB}{3, 79, 132}
\definecolor{iceblue}{RGB}{128, 182, 207}
\definecolor{cc1}{rgb}{0.59, 0.78, 0.64}
\definecolor{niceblue}{RGB}{3, 79, 132}
\definecolor{iceblue}{RGB}{128, 182, 207}
\definecolor{ca3}{rgb}{0.83, 0.69, 0.22}
\definecolor{red1}{RGB}{201,59,69}
\definecolor{red2}{RGB}{169,22,48}
\definecolor{red3}{RGB}{249,129,115}
\definecolor{cl1}{rgb}{0.61, 0.77, 0.89} %nicer lightblue pale cerulean
\definecolor{cl2}{rgb}{0.64, 0.68, 0.82} %lightblue/gray
\definecolor{cl3}{rgb}{0.85, 0.65, 0.13} %nicer goldenrod
\definecolor{ca1}{rgb}{0.6, 0.81, 0.93} %lightblue
\definecolor{ca2}{RGB}{139, 204, 109} %green
% Piglet storyline colours:
\definecolor{rosequartz}{RGB}{247,202,201}
\definecolor{serenity}{RGB}{145,168,209}
\definecolor{peachecho}{RGB}{247,120,107}
\definecolor{snorkelblue}{RGB}{3,79,132}
\definecolor{buttercup}{RGB}{250,224,60}
\definecolor{limpetshell}{RGB}{152,221,222}
\definecolor{lilacgray}{RGB}{152,150,164}
\definecolor{fiesta}{RGB}{221,65,50}
\definecolor{icedcoffee}{RGB}{177,143,106}
\definecolor{greenflash}{RGB}{121,199,83}
\definecolor{purple}{RGB}{153,0,153}
\definecolor{turquise}{RGB}{0,153,153}
\definecolor{poop}{RGB}{203,178,52}
\definecolor{blue1}{RGB}{215, 216, 233}
\definecolor{blue2}{RGB}{243, 243, 248}
\definecolor{varioblue}{RGB}{68, 114, 157}
\definecolor{variogreen}{RGB}{125, 171, 113}
 
\definecolor{slate50}{HTML}{f8fafc} 
\definecolor{slate100}{HTML}{f1f5f9} 
\definecolor{slate200}{HTML}{e2e8f0}
\definecolor{slate300}{HTML}{cbd5e1} 
\definecolor{slate400}{HTML}{94a3b8} 
\definecolor{slate500}{HTML}{64748b} 
\definecolor{cmap1}{RGB}{251,191,36}
\definecolor{cmap2}{RGB}{22,161,74}
\definecolor{cmap3}{RGB}{3,105,161}
\definecolor{cmap4}{RGB}{131,24,76} 

==> sec/background.tex <==
\section{Attribution Methods, formally}
\label{sec:background}
Here we provide a brief formal description of our setting and attribution methods. We consider an input as a vector $x \in \mathcal{I}$, in our setting, the input is typically an image of height $H$, width $W$ and $d$ channels, so $\mathcal{I} = \mathbb{R}^{H \times W \times d}$. We describe a model as a function $S : \mathcal{I} \rightarrow \mathbb{R}^C$, where $C$ is the number of classes in the classification problem. The final classification is usually performed as an argmax over $S(x)$. An attribution method provides a saliency map $\attmap : \mathcal{I} \times S \times \{1,...,C\} \rightarrow \mathcal{I}'$ that for an input, a model, and optionally a target class provides an explanation of the same shape as the input, attributing scores to each feature $i$ in the input describing in how far $S$ uses $x_i$ for the classification (or target class).
Examples of attributions within this definitions could be Input$\times$Gradient (IxG) as $\mathcal{H}_{\text{IxG}}(x, S, c) = x \odot \frac{\partial S_c}{\partial x}$, or
\gradcam as $\mathcal{H}_{\text{\gradcam}}(x, S, c) = \text{ReLU}(\sum_k \alpha_c^k A^k)$, where $\alpha_c^k = \frac{1}{Z} \sum_i \sum_j \frac{\partial S_c}{\partial A_{ij}^k}$ are the importance weights computed by global average pooling of the gradients.




==> tables/pic_comp.tex <==



\begin{wraptable}[14]{r}{0.5\linewidth} % [lines]{l/r}{width}
  \vspace{-\baselineskip}                 % pull up to align with surrounding text
  \centering
  \footnotesize                           % often nicer than resizebox
  \resizebox{\linewidth}{!}{%
    \begin{tabular}{lrrrr}
      \toprule
      & \multicolumn{2}{c}{SIC} & \multicolumn{2}{c}{AIC} \\
      \toprule
      Method & ResNet50 & ViT & ResNet50 & ViT \\
      \midrule
      \gradcam & 0.73 & \textbf{0.54} & 0.76 & \textbf{0.56} \\
      \;w/ \ourmethod & \textbf{0.74} & 0.51 & \textbf{0.78} & 0.52 \\
      \gbpmid & 0.63 & 0.46 & 0.68 & 0.48 \\
      \;w/ \ourmethod & \textbf{0.65} & 0.46 & \textbf{0.70} & 0.48 \\
      \guidedgcfull & 0.69 & \textbf{0.58} & 0.73 & \textbf{0.62} \\
      \;w/ \ourmethod & \textbf{0.7} & 0.52 & \textbf{0.74} & 0.54 \\
      \ixg & 0.52 & \textbf{0.56} & 0.56 & \textbf{0.59} \\
      \;w/ \ourmethod & \textbf{0.53} & 0.51 & \textbf{0.57} & 0.53 \\
      \igfull & 0.56 & 0.55 & 0.60 & 0.57 \\
      \;w/ \ourmethod & \textbf{0.57} & 0.55 & \textbf{0.61} & 0.57 \\
      \bottomrule
    \end{tabular}
  }
  \caption{AIC \& SIC scores for various attribution methods across different models (higher is better).}
  \label{tab:pic}
  \vspace{-\baselineskip}                 % tighten space below
\end{wraptable}

% Your paragraph text naturally flows around the table here...


==> tex_figs/grid/vgg.tex <==

\begin{figure*}
	\begin{tikzpicture}
		\path (0,0) -- (16,0);
		\def\igX{4.2}
		\def\igY{0}
		\node (label_ig) at (\igX, \igY) {\small Integrated Gradients};
		
		\def\gbpX{8.1}
		\def\gbpY{0}
		\node (label_gbp) at (\gbpX, \gbpY) {\small Guided Backprop};
		
		\def\ixgX{12.1}
		\def\ixgY{0}
		\node (label_ixg) at (\ixgX, \ixgY) {\small \ixg};
	\end{tikzpicture}
    \centering
    \includegraphics[width=\linewidth, trim=0 0 0 0, clip]{ICCV2025-Author-Kit/imgs/grid/vgg16_attr_comparison.png} %no clue how this exatcly works
    \caption{\textbf{VGG16}: \textit{\ourmethod on the Grid Pointing Game.} We show examples from the grid pointing game for methods most affected by our framework (as columns: \igfull, \gbpfull, \ixgfull). Input Images are given on the left, for each we provide vanilla attribution methods (top row) and augmented with \ourmethod (bottom row).
    For each, we show the attribution for the four different classes in the grid as columns.}
        \label{app:vgg}
\end{figure*}

